Lost in Translation: Reimagining the Machine Learning Life Cycle in Education

Machine learning (ML) techniques are increasingly prevalent in education, from their use in predicting student dropout, to assisting in university admissions, and facilitating the rise of MOOCs. Given the rapid growth of these novel uses, there is a pressing need to investigate how ML techniques support long-standing education principles and goals. In this work, we shed light on this complex landscape drawing on qualitative insights from interviews with education experts. These interviews comprise in-depth evaluations of ML for education (ML4Ed) papers published in preeminent applied ML conferences over the past decade. Our central research goal is to critically examine how the stated or implied education and societal objectives of these papers are aligned with the ML problems they tackle. That is, to what extent does the technical problem formulation, objectives, approach, and interpretation of results align with the education problem at hand. We find that a cross-disciplinary gap exists and is particularly salient in two parts of the ML life cycle: the formulation of an ML problem from education goals and the translation of predictions to interventions. We use these insights to propose an extended ML life cycle, which may also apply to the use of ML in other domains. Our work joins a growing number of meta-analytical studies across education and ML research, as well as critical analyses of the societal impact of ML. Specifically, it fills a gap between the prevailing technical understanding of machine learning and the perspective of education researchers working with students and in policy.

==> introduction.tex <==
% !TeX root = main.tex 
\section{Introduction}
%\nikhil{Title ideas? ``Strategic ranking, randomized admissions, and student effort'' or current one?}

Many {allocative decisions---from education to employment---}%including {in} allocative settings in which algorithmic solutions have recently played a role {(from} 
%including  across 
%education
 %{to} employment, {to} other settings{)} -- 
 are based not on absolute quality, but rather {relative} quality across individuals: Harvard accepts about 2000 applicants per year, major CS conferences accept about $20\%$ of submissions, and each job opening is filled by one candidate. Even if every applicant improves substantially, the number accepted would not commensurately increase, a reality often rationalized by capacity constraints. The comparative aspect of \textit{ranking} differs sharply from \textit{classification}, in which each entry is evaluated in isolation. %and so if the distribution of features shifts \lledit{due to strategic human behavior}, then so may the distribution of predicted labels.
  While this difference is often overlooked in the machine learning community, we illustrate that {it is consequential and, importantly, motivates \emph{access} as a measure of disparate impact from algorithmic decisions.}%it matters.
%

The specific context of our work is the literature on \textit{strategic classification}, which aims to address gaming (Goodhart’s law) by applicants controlling the classifier's inputs~\cite{Hardt:2016:SC}. For example, if a predictive classifier for admissions learns that a high schooler's number of extracurricular activities correlates with college achievement and thus bases admissions decisions on it, students may sign up for many more activities to list on their applications, without devoting any time to them. A strategic classifier aims to undo this effect, {by shifting weight towards features that are costly to game% and making it more costly to attain a positive classification
	, such that the designer's utility is maximized even taking into account strategic behavior---as in a Stackelberg equilibrium.}%putting more weight on features improved by truly rewarding activities (like studying) and less on those improved by cheating; classifier design becomes a Stackelberg game between the designer and applicants.

Importantly, many motivating applications commonly cited in the strategic classification literature, such as manipulating test scores to gain college admission, are actually ranking problems (or classification with capacity constraints on how many can be classified with each label). This aspect induces competition between applicants, affecting their effort and in turn their comparative performance and ultimate relative position in the ranking. To study the interaction of these effects, this work introduces the problem of \textit{strategic ranking}. 
{We study the general welfare effects of reward design for ranking, and examine the role of randomization in trading off designer's utility and population welfare, as well as reducing disparate impact. This work is complementary to existing work on strategic classification and its welfare implications \citep{hu2019disparate,Milli2019social,braverman2020role}. By shifting our modeling choice from isolation to \emph{competition} between applicants, and our goal from classifier design to \emph{ranking reward design}, we endeavor to fill a gap in the current literature on algorithmic fairness and strategic behavior that has thus far focused on classification, neglecting both these aspects.}
 %Our high level finding is that the change from isolation to competition between applicants substantially changes the insights drawn from the {strategic classification} literature; we study both general welfare effects and in particular the disparate impacts induced both by competition and by the strategic ranking design.  

% As we show \cb{(Christian: I think the competition aspect is obvious, so the we show should apply to something else)}, 

%many strategic classification works motivate their setup with settings more naturally described as a ranking question, especially admissions in education~\todo{cite a few}.

In our strategic ranking framework, a designer ranks applicants by a single, observed measure, called a score. {The score is a function of the applicant's (possibly multi-dimensional) chosen effort level(s), latent skill(s), and environment.} The designer controls the reward $\lambda(\theta)$ assigned to each rank $\theta$, under an overall reward constraint; e.g., in our primary interpretation, the reward is a probability at which an applicant of each rank is admitted. In response, the applicants choose their (costly) {effort level} for the observed measure, such that in equilibrium{---that is, given the effort levels of the entire applicant population---}their effort level and resulting rank maximizes their welfare (reward minus effort cost). Depending {on} the setting, the designer's objective may be a function of applicant effort and who is admitted. Using this model, our contributions are as follows.

\textbf{First}, we analyze the equilibrium behavior and resulting optimal designs, illuminating important differences between the classification and ranking settings. We show that, in a general setting and with any reasonable reward function $\lambda$, the competition effect results in \textit{rank preservation}: in equilibrium, the ranks (and thus rewards) of applicants after applicant effort is the same as before. This finding differs from strategic classification -- where one must adapt to the effort it induces to maintain accuracy~\cite{Hardt:2016:SC} -- and simplifies subsequent equilibrium analysis.

\textbf{Second}, we study how the design of reward function $\lambda$ differentially affects the welfare of various stakeholders: applicants, a school preferring to admit those with the highest score, and a social planner maximizing the score over the population. We find, for example, there is an interesting trade-off even in one skill dimension: while deterministically admitting the highest ranked students may maximize the school's utility, it leads to applicants exerting costly effort. Adding randomness reduces pressure for applicants at the expense of the school's utility. 

\textbf{Third}, we analyze equilibria in the presence of structural inequities between different groups, finding that competition amplifies such inequities without careful reward design: designing reward $\lambda$ to increasing school utility increases the welfare gap between groups, and decreases \textit{access} (group specific admission probabilities) for the disadvantaged group.

We note that our research questions are strongly influenced by analogous questions in the strategic classification literature. However, unlike strategic classification, which focuses on unproductive gaming, our model considers applicants who compete in a meaningful measure of skill. Our framework allows for direct comparisons of participant welfare at a societal level, beyond ``narrowly bracketed'' notions of algorithmic fairness, as, e.g., recently advocated by~\citet{kasy2021fairness}. In addition, our definitions of school utility and group access---while natural for constrained allocation settings---cannot be studied in unconstrained classification settings, where policies may admit different numbers of applicants.





% \lnote{Nikhil to do a writing pass for Contributions:}
% \begin{enumerate}
% 	\item equilibrium characterization - second price effort. ranking is preserved if there are no environmental differences.
% 	\item welfare tradeoffs - emphasize different stakeholders/utility v.s. welfare, reward design (level of randomization). tension between designer and population benefit have been observed in strategic classification as well - (we consider the additional measure of "societal utility", which is distinct from economic notion of social welfare.)
% 	\item  Disparate impact: Extend our equilibrium analysis to when there are environmental differences. We find that Structural inequalities are amplified by competition - increasing the school's private utility increases the welfare gap, and decreases access. * Access (as defined as overall probability of admission for the disadvantaged group) is an aspect that has not been studied in the strategic classification literature, which has focused on the disparate costs of manipulation. However, in the competitive/resource-constrained setting, the loss of access is arguably as significant as disparate costs.
% 	\item multi-dimensional competition - ? (figure out what the takeaway is) extension/multi-dimensional analogue in appendix.
% \end{enumerate}}



% \nikhil{I think rewrite this, to emphasize welfare differences based on who is deciding $\lambda$ -- make that part of the access/equity thing}While the design of $\lambda$ does not influence the final ranking, it does affect the utility of students (whose effort level to maintain their rank depends on $\lambda$) and {of} the designer, who may care about the post-effort skill levels of those it admits. We note %CB: here 
% that in our model, there is an interesting trade-off even in one skill dimension: if the school deterministically admits the highest ranked students, then its utility is maximized, while students may be exerting costly, ultimately meaningless effort. Adding randomness reduces pressure for students at the expense of the school's utility.

% \todo{(Christian: we should somewhere before this sentence say that we may be one-dimension, or multi-dimensional)}



%\nikhil{First, Insights change in a ranking context -- In ranking, competition between agents, who can put effort in to increase their features, could undo the classification aspect. In our main result, rankings remain the same according to some pre-index…very general model, etc....also interesting in single dimension
%}
%
%\nikhil{Second, ranking allows us to compare different objectives, like value of those admitted vs overall. The equivalent notions are difficult to do in classification ---- hmm, is this worth it in the introduction?
%}
% \nikhil{From Christian -- Below is not quite good yet, not fluent yet}




% Finally, we extend our analysis to a multi-dimensional setting in which students can exert effort to increase multiple features; reward design influences the distribution of effort across features.%However, one feature is unobservable.


% \nikhil{"Extensions"
% 	1. Environment --- related to equity
% 2. Measurability of features}

% This competition between applicants induces a strategic aspect to ranking problems

% Rankings thus induce competition between applicants

%\todo{notes re contribution:}
%\begin{itemize}
%    \item We introduce the strategic ranking problem, and show how equilibrium behavior and corresponding design insights may differ substantially from strategic classification. \todo{draw out differences with strategic classification}
%
%
%
%    \item randomized admissions policies
%
%
%    \item measurability of features/combining `useful' and 'gaming' -- opportunity costs
%
%    \item     Using our framework, we further study disparate impacts of strategic ranking, finding that \todo{}.
%
%        \item comparison to one-dim strategic classification? something crisp/meaningful about the difference / what the capacitated setting captures. e.g. not well defined to compare FN and FP in a setting where different models select different numbers of positives.
%
%\end{itemize}


%\nikhil{unique combination in this work:}
%\begin{itemize}
%    \item effort can be productive, but also too much (hurt other dimension)
%    \item Design of
%\end{itemize}

\vspace{.5em}
The paper is organized as follows. \Cref{sec:modelequil} contains our model and an analysis of the induced equilibrium. In \Cref{sec:welfare} we analyze how who chooses $\lambda$ affects the welfare of applicants, the school, and society. \Cref{sec:environment} focuses on disparate impacts of strategic ranking with heterogeneous access to resources. We conclude in Section~\ref{sec:conclusion} by briefly outlining an agenda in strategic ranking.  In \Cref{sec:multi-dim} we extend our model to a multi-dimensional setting.  All proofs are in the Appendix. 

%\lnote{Strategic classification views the cost of exerting effort to change one's features, such as SAT scores, as unrelated to one's underlying merit. Our first main result, on the other hand, shows that as long as one's `cost' is monotonically decreasing in merit, then the fact that individuals can strategize on their features does not change the pool of individuals selected. }

\input{related}

==> related.tex <==
\subsection*{Related work}
Our work sits at the intersection of work in two communities,
\textit{strategic classification} and \textit{fair machine learning} in computer science, and \textit{contests} and \textit{effort} in economics. %\nikhil{3 audiences -- classification, FATE, economics}
%
In developing a framework for strategic ranking, we primarily contrast with the main findings of the \textit{strategic classification} literature, demonstrating how a simple change from the classification to the ranking setting changes many insights. Our analyses are also motivated by recent work considering equity in allocation and ranking problems. In pursuit of these questions, our theoretical framework borrows from the economics literature on \textit{contests}, in which agents expend effort to obtain a reward that is a function of their relative performance across agents.

%\footnote{equivalently, binary classification to constrained binary classification holding constant the number of positive labels}

%\nikhil{From Christian -- less defending of work from econ audience, speak more to CS audience and be honest about what we get from the econ audience. Maybe be even more explicit about it, relate to the FATE community more}


% Our work is at the intersection of two literatures that consider these effects.  As in ranking contests \nikhil{wc?}, in our model agents are further incentivized by competition from other agents. We show how the two effects interact, and how the challenge of accurately ranking agents is complicated by needing to incentivize productive effort.

\parbold{Strategic classification} As in strategic classification~\cite{Hardt:2016:SC,miller2020strategic}, we consider the challenge an institution faces when deploying a classifier that applicants can game; a naive classifier that does not factor in the resulting distribution shifts would be inaccurate. Unlike strategic classification, which considers the manipulation of observable features to be entirely unproductive from the institution's perspective, our model of efforts stipulates that the school prefers higher effort levels as they give rise to higher scores.  We follow the line of work considering the design of reward functions that further incentivize agent effort on productive tasks~\cite{kleinberg18investeffort}.

We in particular draw inspiration from and compare to several recent directions in the strategic classification literature: with multiple agents, when a classifier may be random, and with fairness concerns.~\citet{haghtalab2020maximizing} and~\citet{alon2020multiagent} both study multi-agent strategic classification where the principal's goal is to incentiv{ize} %e
% 
agents to improve their features in a productive manner (as opposed to, e.g., cheating); in our setting, the different agents may have different initial features and cost functions, but also impose competitive pressures on each other. \citet{hu2019disparate} and \citet{Milli2019social} consider the (potentially heterogeneous) cost of strategic classification on applicants, as in equilibrium (due to the classifier's adjustment) they must exert extra effort to be admitted. In our model with disparate costs, a student from the disadvantaged group similarly must exert a greater effort to be admitted than a student from the advantaged group, and this effort differential worsens with increased competition. Finally, \citet{braverman2020role} study the role of randomized classifiers and noisy features in strategic classification, showing that a randomized classifier can prevent  undesirable strategic behavior {by an applicant}; they further show that \textit{after} applicants have responded to a randomized classifier, randomization is not a best response for the institution. It is also shown that noisy features can reduce disparate impact when there are two subpopulations with different costs of manipulation. In our setting, randomization (after applicants have been ranked) plays three roles: to prevent strategic behavior at the cost of other, less measurable beneficial features, to lessen competitive pressure, and to increase fairness in the presence of disparate costs. %In our setting, we find that using a randomized decision policy could be justified by social welfare objectives or when there is a unmeasurable attribute.

Like other strategic classification work, our work is further related to the prior economics literature on contract design. In particular, one of our multidimensional extensions is directly motivated by the classic contract design work of~\citet{holmstrom1991multitask}, who show that when some work tasks are less measurable than others, it may be optimal to lessen incentives on the measurable tasks (e.g., by adopting a fixed wage) so as to not crowd out effort in the less measurable ones. In our multidimensional setting, the college faces similar tradeoffs, with the additional challenge that it now must rank multiple applicants. % \todo{other contract design}
%Most related is the work of


\parbold{Economics: Contests and modeling effort} Our theoretical analysis is similar to that in the literature on \textit{contests} in economics~\cite{barut1998symmetric}; e.g., our rank preservation result in \Cref{sec:equillemmas} reflects assortative allocation results in the literature under similar conditions. The field is too extensive to summarize here, so we refer the reader to surveys~\cite{corchon2007theory,fu2019contests} and discuss the works closest to ours.

\citet{bodoh2018college} develop a model with heterogeneous students endogenously choosing effort in an admissions game; they use the model to compare various affirmative action schemes. \citet{fang2020turning} find that increased competition (in form of either more contestants or more convex reward structure) decreases overall student effort. Most related is the line of work by~\citet{olszewski2016large,olszewski2019bid,olszewski2019pareto}. \citet{olszewski2019pareto} find that policies that ``pool'' individuals into tiers (as opposed to continuous ranks) can be Pareto improving for students, as even those with decreased individual rewards would benefit from decreased competitive pressure. 

Our work departs from the contests literature through its focus on the questions most common in the strategic classification literature: while the contests literature primarily considers the efforts and resulting welfare of participants, we study how the design of the reward function $\lambda$ differentially affects the corresponding designer's utility, applicant welfare, and fairness metrics. In particular, when $\lambda$ is interpreted as a probability of admission, our designer faces tradeoffs with incentivizing overall effort and admitting the most skilled students (\Cref{sec:welfare}); with disparate access, the designer must further navigate trade-offs between fairness and inducing effort (\Cref{sec:environment}); with multiple score dimensions, the designer must ensure that applicants do not excessively game one dimension at the cost of the other (\Cref{sec:multi-dim}). Simultaneous to us, \citet{elkind2021contest} consider the effect of contest design on participant and designer welfare. 

Beyond the contests literature, our work connects to the economics literature on student effort and subsequent reward. We incorporate two well-studied rewards from effort: a signal of one's quality in a competition~\cite{spence1978job} (in our model, the incentive of students), and productive development of human capital~\cite{becker1973theory} (in our model, the goal of the school). Following \citet{roemer1998equality}, \citet{calsamiglia09decent} considers a model in which measurable performance in a competitive activity is a product of effort, a relevant characteristic (such as academic talent), and an irrelevant characteristic (such as proximity to a library); the work studies mechanisms to achieve global equality of opportunity---in which students' post-allocation welfare does not depend on irrelevant characteristics---when allocations are determined locally for each competitive activity, e.g., the NBA and college admissions.
% \todo{where does this go? Lydia is this that paper that you were looking at earlier?}
%  \lnote{Yes. I added a blurb. }
% \lnote{This would fall under the line of work on equality of opportunity, which formalized the concept of effort etc. }




\parbold{FATE in machine learning and MD4SG} Finally, we broadly connect to the Fairness, Accessibility/Accountability, Transparency, and Ethics (FATE) in machine learning \cite{Chouldechova2018TheFO} and the Mechanism Design for Social Good (MD4SG) literatures \cite{abebe2018mechanism}. Most relevant are works on fair ranking, constrained allocation, and admissions. The fair allocation literature also considers the allocation of (often indivisible) resources in a budgeted setting, with various fairness notions defined at the group or individual level~\cite{aziz2020developments,caifair2020,golz2019paradoxes,noriega2019active}---such as when one group due to external discrimination faces a disadvantage in features. Similarly, fair ranking works consider the distribution of ranking slots to agents who belong to various groups~\cite{mathioudakis2020affirmative,zehlike2017fa,zehlike2020reducing} or to items that each have a certain social utility \cite{tabibian2020design}. In both settings, the mechanism designer must balance allocation based on ``relevance'' with an appropriate fairness notion. Finally, the burgeoning mechanism design literature on fair admissions (and more generally, classification) considers the design of mechanisms that can counter historic and ongoing inequities~\cite{faenza2020impact,garg2020dropping,immorlica2019access,kannan2021best,liu2020disparate,Hu2018shortterm,Mouzannar2019socialequality,kannan2019downstream,liu2018delayed,rolf2020balancing,liu2021test}. In this work (and especially in \Cref{sec:environment}), we consider such effects as they interact with agents' strategic responses to the mechanism.

%Finally, our work is part of the burgeoning , which considers the design of mechanisms 
%Much of the fair allocation literature studies information acquisition policies by the school, without considering agents' strategic responses \cite{aziz2020developments}.~\citet{noriega2019active} and \citet{caifair2020}, for example, also consider various fairness notions in a budgeted setting, when the school can acquire additional information on applicants. 








%\todo{include citations to fair ML work in education/allocation in general, to the community that will read this paper} ~\cite{,} 

% \nikhil{include your works too here, Lydia!}

%\cite{liu2020disparate,Hu2018shortterm,Mouzannar2019socialequality,kannan2019downstream} dynamics of decision making and ramifications for fairness.
%
%\cite{liu2018delayed, rolf2020balancing} considered multiple objectives.
